A Stable Cardinality Distance for Topological Classification

This work incorporates topological features via persistence diagrams to classify point cloud data arising from materials science. Persistence diagrams are multisets summarizing the connectedness and holes of given data. A new distance on the space of persistence diagrams generates relevant input features for a classification algorithm for materials science data. This distance measures the similarity of persistence diagrams using the cost of matching points and a regularization term corresponding to cardinality differences between diagrams. Establishing stability properties of this distance provides theoretical justification for the use of the distance in comparisons of such diagrams. The classification scheme succeeds in determining the crystal structure of materials on noisy and sparse data retrieved from synthetic atom probe tomography experiments.

==> draft v4a/tex/shared.tex <==
\NeedsTeXFormat{LaTeX2e}
\usepackage{newtxtext,newtxmath}       % selects Times Roman as basic font
\usepackage{helvet}         % selects Helvetica as sans-serif font
\usepackage{courier}        % selects Courier as typewriter font
%\usepackage{type1cm}        % activate if the above 3 fonts are not available on your system
%\usepackage{makeidx}         % allows index generation
\usepackage{graphicx}        % standard LaTeX graphics tool
\usepackage{multicol}        % used for the two-column index
\usepackage[bottom]{footmisc}% places footnotes at page bottom
\usepackage{amsmath,amssymb, amsfonts, mathtools}       % AMS math packages
\usepackage{verbatim, booktabs}
\usepackage{bbm, bm}
\usepackage{wrapfig}
%\usepackage{caption}
\usepackage[capitalise]{cleveref}
\usepackage{chngcntr}
\usepackage{apptools}
%\usepackage{lineno}
%\usepackage{showkeys}
% see the list of further useful packages in the Reference Guide
%\makeindex             % used for the subject index

% uncomment this to show line numbers
%\linenumbers

% algorithm title
%\Crefformat{figure}{#2{}{Figure}~#1{}#3}
\crefdefaultlabelformat{#2{\scshape #1}#3}

\usepackage{subcaption}
\captionsetup{compatibility=false}
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{varwidth}
%\usepackage{algorithmic}
%\usepackage{algorithm}
\usepackage{color, booktabs}
\usepackage[table]{xcolor}

\usepackage{tabularx}
\usepackage[export]{adjustbox}


\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Ind}{\mathbbm{1}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\Var}{\mathrm{Var}}
\DeclareMathOperator{\diag}{diag}
\newcommand{\dpc}{d_p^c}
% \renewcommand{\qed}{\hfill\blacksquare}

\newcommand{\todoC}[1]{{\color{purple}{#1}}}
\newcommand{\todoA}[1]{{\color{red}{#1}}}
\newcommand{\revision}[1]{{\color{blue}{#1}}}
\newcommand{\rev}[1]{{\color{blue}{#1}}}

\newtheorem{thm}{Theorem}
\newtheorem{theorem}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{pf}{Proof}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{definition}[thm]{Definition}

\newcommand{\proofofref}{}
\newtheorem{zproofof}{Proof of \proofofref}
\newenvironment{pot}[1]
{\renewcommand{\proofofref}{#1}\zproofof}
{\endzproofof}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\ifpdf
\DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
\DeclareGraphicsExtensions{.eps}
\fi

\newcommand{\creflastconjunction}{, and~}

==> tex/shared.tex <==
\NeedsTeXFormat{LaTeX2e}
\usepackage{newtxtext,newtxmath}       % selects Times Roman as basic font
\usepackage{helvet}         % selects Helvetica as sans-serif font
\usepackage{courier}        % selects Courier as typewriter font
%\usepackage{type1cm}        % activate if the above 3 fonts are not available on your system
%\usepackage{makeidx}         % allows index generation
\usepackage{graphicx}        % standard LaTeX graphics tool
\usepackage{multicol}        % used for the two-column index
\usepackage[bottom]{footmisc}% places footnotes at page bottom
\usepackage{amsmath,amssymb, amsfonts, mathtools}       % AMS math packages
\usepackage{verbatim, booktabs}
\usepackage{bbm, bm}
\usepackage{wrapfig}
%\usepackage{caption}
\usepackage[capitalise]{cleveref}
\usepackage{chngcntr}
\usepackage{apptools}
%\usepackage{lineno}
%\usepackage{showkeys}
% see the list of further useful packages in the Reference Guide
%\makeindex             % used for the subject index

% uncomment this to show line numbers
%\linenumbers

% algorithm title
%\Crefformat{figure}{#2{}{Figure}~#1{}#3}
\crefdefaultlabelformat{#2{\scshape #1}#3}

\usepackage{subcaption}
\captionsetup{compatibility=false}
\usepackage{enumitem}
\usepackage{epstopdf}
\usepackage{varwidth}
%\usepackage{algorithmic}
%\usepackage{algorithm}
\usepackage{color, booktabs}
\usepackage[table]{xcolor}

\usepackage{tabularx}
\usepackage[export]{adjustbox}


\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Ind}{\mathbbm{1}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\Var}{\mathrm{Var}}
\DeclareMathOperator{\diag}{diag}
\newcommand{\dpc}{d_p^c}
% \renewcommand{\qed}{\hfill\blacksquare}

\newcommand{\todoC}[1]{{\color{purple}{#1}}}
\newcommand{\todoA}[1]{{\color{red}{#1}}}
\newcommand{\revision}[1]{{\color{blue}{#1}}}
\newcommand{\rev}[1]{{\color{blue}{#1}}}

\newtheorem{thm}{Theorem}
\newtheorem{theorem}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{pf}{Proof}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{definition}[thm]{Definition}

\newcommand{\proofofref}{}
\newtheorem{zproofof}{Proof of \proofofref}
\newenvironment{pot}[1]
{\renewcommand{\proofofref}{#1}\zproofof}
{\endzproofof}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\ifpdf
\DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
\DeclareGraphicsExtensions{.eps}
\fi

\newcommand{\creflastconjunction}{, and~}
